Efficient and Effective Tail Latency Minimization in Multi-Stage Retrieval Systems

Scalable web search systems typically employ multi-stage retrieval architectures, where an initial stage generates a set of candidate documents that are then pruned and re-ranked. Since subsequent stages typically exploit a multitude of features of varying costs using machine-learned models, reducing the number of documents that are considered at each stage improves latency. In this work, we propose and validate a unified framework that can be used to predict a wide range of performance-sensitive parameters which minimize effectiveness loss, while simultaneously minimizing query latency, across all stages of a multi-stage search architecture. Furthermore, our framework can be easily applied in large-scale IR systems, can be trained without explicitly requiring relevance judgments, and can target a variety of different efficiency-effectiveness trade-offs, making it well suited to a wide range of search scenarios. Our results show that we can reliably predict a number of different parameters on a per-query basis, while simultaneously detecting and minimizing the likelihood of tail-latency queries that exceed a pre-specified performance budget. As a proof of concept, we use the prediction framework to help alleviate the problem of tail-latency queries in early stage retrieval. On the standard ClueWeb09B collection and 31k queries, we show that our new hybrid system can reliably achieve a maximum query time of 200 ms with a 99.99% response time guarantee without a significant loss in overall effectiveness. The solutions presented are practical, and can easily be used in large-scale distributed search engine deployments with a small amount of additional overhead.

==> pipeline2.tex <==
\begin{algorithm}
    \SetKwInOut{Input}{Input}
    \SetKwInOut{Output}{Output}

\caption{Candidate generation pipeline based on predicting the query runtime $t$}
%{\bf Input:}\\
\Input{A query $q$, a regressor $\mathcal{R}_k$ that predicts the required $k$, 
	a regressor $\mathcal{R}_\rho$ that predicts the required $\rho$ for \jass{}, 
a run-time regressor $\mathcal{R}_t$, and runtime-threshold $T_t$}
\Output{A set of candidate documents, $C$}
$C = \{\}$\\
$P_k = \mathcal{R}_k(q)$\\
$P_t = \mathcal{R}_t(q)$\\
\eIf{$P_t > T_t$}
{
  $P_\rho = \mathcal{R}_\rho(q)$\\
  $C = $ \jass{}$(q, P_k, P_\rho)$\\
}
{
  $C = $ \bmw{}$(q, P_k)$\\
}
return $C$
\end{algorithm}


